RACE: RoPE-Aligned Attention Compression Based on Query-Key Activation Energies

Head-dimension compression can reduce the memory required by the key-value (KV) cache, but existing methods often reconstruct full-dimensional representations during inference, adding significant decoding FLOPs overhead. We formalize the design considerations for converting pretrained attention into a natively reduced-dimensional form that reduces both KV-cache storage and attention computation using a calibration set. Specifically, we consider reductions that (1) apply a shared projection to queries and keys so that they remain in a common reduced feature space, (2) derive this projection jointly from query and key activations to better preserve their interaction, and (3) are compatible with the pretrained RoPE transformation. To obtain a reconstruction-free realization of this reduction, we restrict it to coordinate selection and theoretically show that RoPE compatibility then holds if and only if complete rotary pairs are retained. Building on this characterization, we introduce RACE, a post-training method that selects rotary pairs using their joint query-key activation energy. We theoretically show that this criterion minimizes a separable, calibration-dependent upper bound on post-RoPE query-key product approximation error. The resulting reductions are folded into the model weights and require neither runtime reconstruction nor specialized kernels. Across three model families and different compression levels, RACE outperforms structured pruning and remains competitive with reconstruction-based methods on language-modeling, zero-shot, and long-context tasks. At 50% KV-cache retention and 256K context, RACE reduces total inference FLOPs by 47.8%, yielding 1.79x higher throughput, 43.2% lower time-to-first-token (TTFT), and 28.1% lower allocated GPU memory in comparison to an uncompressed model.

==> tables/FLOPs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% \usepackage{graphicx}

\begin{table}[t]
\caption{
\textbf{Cache-length-dependent decoding arithmetic at representative KV Cache compression.}
We report arithmetic terms that scale with cache length $S$ during autoregressive decoding. We use $H_q=H_{\mathrm{kv}}=6$, $d_k=d_v=128$, and
$r_k=r_v=64$ for EigenAttention and Ours. For the PALU G-LRD calculation, we use $G=3$ groups and $r_k^{G}=r_v^{G}=128$, yielding 50\% KV Cache compression. For Thin Keys, we use $r_k= 64; r_v=128$ as it does not support V compression. Full FLOPs analysis is given in Appendix \ref{app:flops_analysis}
}
\vspace{0.25cm}
\label{tab:flops}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\hline

\rowcolor[HTML]{EFEFEF}
\textbf{Method}
&
\begin{tabular}[c]{@{}c@{}}
\textbf{KV Cache}\\
\textbf{Retained}
\end{tabular}
&
\begin{tabular}[c]{@{}c@{}}
\textbf{$S$-dependent Arithmetic}\\
\textbf{per Decode Step}
\end{tabular}
&
\begin{tabular}[c]{@{}c@{}}
\textbf{Relative}\\
\textbf{$S$-dependent Arithmetic}
\end{tabular}
\\
\hline

Full Attention
&
$100\%$
&
$\mathcal{O}\!\left(BSH_q(d_k+d_v)\right)$
&
$1.00\times$
\\

\rowcolor[HTML]{EFEFEF}
EigenAttention~\cite{saxena2024eigen}
&
$50\%$
&
$\mathcal{O}\!\left(
BS\left[
H_{\mathrm{kv}}r_kd_k+
H_q(d_k+r_v)
\right]
\right)$
&
$32.75\times$
\\

PALU (G-LRD)~\cite{chang2025palu}
&
$50\%$
&
$\mathcal{O}\!\left(
BS\left[
H_{\mathrm{kv}}r_k^{G}d_k+
H_qd_k+Gr_v^{G}
\right]
\right)$
&
$64.75\times$
\\

\rowcolor[HTML]{EFEFEF}
Thin Keys Full Values~\cite{thinkeys}
&
$75\%$
&
$\mathcal{O}\!\left(
BSH_q(r_k+d_v)
\right)$
&
$0.75\times$
\\

\textbf{Ours}
&
\textbf{$50\%$}
&
$\mathbf{
\mathcal{O}\!\left(
BSH_q(r_k+r_v)
\right)
}$
&
$\mathbf{0.50\times}$
\\

\hline
\end{tabular}
}


\vspace{0.05cm}


\end{table}

==> tables/additional_complementary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{
}
% \vspace{0.25cm}
\label{tab:add_complementary}
\centering
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{ccccccccccccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Method}                                                      &  & \multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{H2O: KV Size 256}} & \textbf{} & \multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{SnapKV: KV Size 256}} & \textbf{} & \multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{KIVI 2 bits}} \\
\textbf{\begin{tabular}[c]{@{}c@{}}Head Dim\\ Retained\end{tabular}} &  & 100\%                 & 75\%                  & 50\%                  &           & 100\%                  & 75\%                   & 50\%                   &           & 100\%                & 75\%                & 50\%                \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{wikitext (ppl)}    &  & 13.62                 & 15.12                 & 21.81                 &           & 12.76                  & 15.66                  & 18.44                  &           & 15.7                 & 16.58               & 17.14               \\
\textbf{hellaswag}                                                       &  & 0.66                  & 0.65                  & 0.62                  &           & 0.68                   & 0.65                   & 0.62                   &           & 0.69                 & 0.66                & 0.64                \\
\rowcolor[HTML]{EFEFEF} 
\textbf{piqa}                                                        &  & 0.85                  & 0.83                  & 0.79                  &           & 0.85                   & 0.83                   & 0.79                   &           & 0.86                 & 0.84                & 0.8                 \\
\textbf{arc\_challenge}                                                      &  & 0.48                  & 0.45                  & 0.42                  &           & 0.48                   & 0.45                   & 0.46                   &           & 0.48                 & 0.48                & 0.44                \\
\rowcolor[HTML]{EFEFEF} 
\textbf{boolq}                                                       &  & 0.79                  & 0.78                  & 0.71                  &           & 0.81                   & 0.79                   & 0.74                   &           & 0.78                 & 0.78                & 0.74                \\
\textbf{MMLU College CS}      &  & 0.66                  & 0.63                  & 0.4                   &           & 0.7                    & 0.63                   & 0.44                   &           & 0.7                  & 0.63                & 0.42                \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Avg Acc}                                                     &  & 0.688                 & 0.668                 & 0.588                 &           & 0.704                  & 0.67                   & 0.61                   &           & 0.7                  & 0.63                & 0.42                \\ \hline
\end{tabular}
}
\end{table}

==> tables/main_ZS.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{\textbf{Best-performing configuration at each KV-cache compression
level.} For each method, model, and cache-retention level, we report the
$(r_k,r_v)$ configuration with the highest average downstream accuracy at the same cache size. Each category column averages the
tasks belonging to that category, and \emph{Average} is computed across all
downstream tasks. The complete results for every $(r_k,r_v)$ configuration,
individual tasks, and more baseline methods are provided in Table ~\ref{tab:ZS_full}.}
\label{tab:main_ZS}
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{cccccccccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Method}                                                                      & \rothead{\textbf{\begin{tabular}[c]{@{}c@{}}KV Cache\\ Retained\end{tabular}}} & \rothead{\textbf{\begin{tabular}[c]{@{}c@{}}Wikitext\\ (ppl)\end{tabular}}} & \rothead{\textbf{\begin{tabular}[c]{@{}c@{}}Comple-\\ tion\end{tabular}}}                              & \rothead{\textbf{\begin{tabular}[c]{@{}c@{}}Reaso-\\ ning\end{tabular}}}           & \rothead{\textbf{\begin{tabular}[c]{@{}c@{}}Knowle-\\  dge \& QA\end{tabular}} }& \rothead{\textbf{\begin{tabular}[c]{@{}c@{}}Unders-\\ tanding\end{tabular}}}        & \rothead{\textbf{\begin{tabular}[c]{@{}c@{}}Truth-\\ fulness\end{tabular}}}         & \rothead{\textbf{\begin{tabular}[c]{@{}c@{}}Specialized \\ Knowledge\end{tabular}}} & \rothead{\textbf{Avg.} }             \\ \hline
\multicolumn{10}{c}{\textbf{Qwen2.5 7B}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\textbf{Base}                                                                        & \cellcolor[HTML]{EFEFEF}100\%                                        & \cellcolor[HTML]{EFEFEF}10.976                                    & \cellcolor[HTML]{EFEFEF}0.706                     & \cellcolor[HTML]{EFEFEF}0.761 & \cellcolor[HTML]{EFEFEF}0.572                                       & \cellcolor[HTML]{EFEFEF}0.632 & \cellcolor[HTML]{EFEFEF}0.524 & \cellcolor[HTML]{EFEFEF}0.652                                             & \cellcolor[HTML]{EFEFEF}0.671 \\ \hdashline
                                                                                     & 75\%                                                                 & 11.325                                                            & 0.695                                             & 0.766                         & 0.653                                                               & 0.631                         & 0.532                         & 0.628                                                                     & 0.668                         \\
\multirow{-2}{*}{\textbf{PALU}}                                                      & \cellcolor[HTML]{EFEFEF}50\%                                         & \cellcolor[HTML]{EFEFEF}17.240                                    & \cellcolor[HTML]{EFEFEF}0.639                     & \cellcolor[HTML]{EFEFEF}0.699 & \cellcolor[HTML]{EFEFEF}0.595                                       & \cellcolor[HTML]{EFEFEF}0.591 & \cellcolor[HTML]{EFEFEF}0.430 & \cellcolor[HTML]{EFEFEF}0.559                                             & \cellcolor[HTML]{EFEFEF}0.605 \\ \hdashline
                                                                                     & 75\%                                                                 & 10.080                                                            & 0.715                                             & 0.753                         & 0.635                                                               & 0.613                         & 0.545                         & 0.616                                                                     & 0.658                         \\

\multirow{-2}{*}{\textbf{RAP}}                                                       & 50\%                                                                 & 14.691                                                            & 0.485                                             & 0.704                         & 0.596                                                               & 0.549                         & 0.403                         & 0.411                                                                     & 0.549                         \\ \hdashline
                                                                                     & \cellcolor[HTML]{EFEFEF}75\%                                         & \cellcolor[HTML]{EFEFEF}10.916                                    & \cellcolor[HTML]{EFEFEF}0.690                     & \cellcolor[HTML]{EFEFEF}0.759 & \cellcolor[HTML]{EFEFEF}0.640                                       & \cellcolor[HTML]{EFEFEF}0.613 & \cellcolor[HTML]{EFEFEF}0.521 & \cellcolor[HTML]{EFEFEF}0.628                                             & \cellcolor[HTML]{EFEFEF}0.661 \\
\multirow{-2}{*}{\textbf{Ours}}                                                      & 50\%                                                                 & 13.538                                                            & 0.562                                             & 0.726                         & 0.619                                                               & 0.577                         & 0.464                         & 0.515                                                                     & 0.600                         \\ \hline
\multicolumn{10}{c}{\textbf{Granite 4.1 3B}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \hline
\textbf{Base}                                                                        & \cellcolor[HTML]{EFEFEF}100\%                                        & \cellcolor[HTML]{EFEFEF}11.578                                    & \cellcolor[HTML]{EFEFEF}0.662                     & \cellcolor[HTML]{EFEFEF}0.757 & \cellcolor[HTML]{EFEFEF}0.633                                       & \cellcolor[HTML]{EFEFEF}0.558 & \cellcolor[HTML]{EFEFEF}0.476 & \cellcolor[HTML]{EFEFEF}0.564                                             & \cellcolor[HTML]{EFEFEF}0.629 \\ \hdashline
                                                                                     & 75\%                                                                 & 11.918                                                            & 0.675                         & 0.750                        &                  0.628                                              &           0.562               &        0.468                   &                       0.568                                              & 0.628                         \\
\multirow{-2}{*}{\textbf{PALU}}                                                      & \cellcolor[HTML]{EFEFEF}50\%                                         & \cellcolor[HTML]{EFEFEF}17.483                                    & \cellcolor[HTML]{EFEFEF}0.539 & \cellcolor[HTML]{EFEFEF}0.671   & \cellcolor[HTML]{EFEFEF}   0.590                                  & \cellcolor[HTML]{EFEFEF}0.535 & \cellcolor[HTML]{EFEFEF}0.456   & \cellcolor[HTML]{EFEFEF}     0.437                                      & \cellcolor[HTML]{EFEFEF}0.551 \\ \hdashline
                                                                                     & 75\%                                                                 & 13.993                                                            & 0.577                                             & 0.730                         & 0.627                                                               & 0.553                         & 0.440                         & 0.526                                                                     & 0.602                         \\

\multirow{-2}{*}{\textbf{RAP}}                                                       & 50\%                                                                 & 17.766                                                            & 0.359                                             & 0.653                         & 0.556                                                               & 0.474                         & 0.405                         & 0.225                                                                     & 0.460                         \\ \hdashline
                                                                                     & \cellcolor[HTML]{EFEFEF}75\%                                         & \cellcolor[HTML]{EFEFEF}13.148                                    & \cellcolor[HTML]{EFEFEF}0.611                     & \cellcolor[HTML]{EFEFEF}0.737 & \cellcolor[HTML]{EFEFEF}0.624                                       & \cellcolor[HTML]{EFEFEF}0.545 & \cellcolor[HTML]{EFEFEF}0.441 & \cellcolor[HTML]{EFEFEF}0.537                                             & \cellcolor[HTML]{EFEFEF}0.607 \\
\multirow{-2}{*}{\textbf{Ours}}                                                      & 50\%                                                                 & 16.210                                                            & 0.516                                             & 0.669                         & 0.584                                                               & 0.510                         & 0.462                         & 0.405                                                                     & 0.537                         \\ \hline
\multicolumn{10}{c}{\textbf{Llama 3.2 3B Instruct}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\textbf{Base}                                                                        & \cellcolor[HTML]{EFEFEF}100\%                                        & \cellcolor[HTML]{EFEFEF}13.397                                    & \cellcolor[HTML]{EFEFEF}0.659                     & \cellcolor[HTML]{EFEFEF}0.706 & \cellcolor[HTML]{EFEFEF}0.584                                       & \cellcolor[HTML]{EFEFEF}0.597 & \cellcolor[HTML]{EFEFEF}0.496 & \cellcolor[HTML]{EFEFEF}0.514                                             & \cellcolor[HTML]{EFEFEF}0.599 \\ \hdashline
                                                                                     & 75\%                                                                 & 14.719                                                            & 0.637                                             & 0.688                         & 0.584                                                               & 0.594                         & 0.446                         & 0.500                                                                     & 0.583                         \\
\multirow{-2}{*}{\textbf{PALU}}                                                      & \cellcolor[HTML]{EFEFEF}50\%                                         & \cellcolor[HTML]{EFEFEF}22.435                                    & \cellcolor[HTML]{EFEFEF}0.543                     & \cellcolor[HTML]{EFEFEF}0.629 & \cellcolor[HTML]{EFEFEF}0.540                                       & \cellcolor[HTML]{EFEFEF}0.567 & \cellcolor[HTML]{EFEFEF}0.440 & \cellcolor[HTML]{EFEFEF}0.395                                             & \cellcolor[HTML]{EFEFEF}0.522 \\ \hdashline
                                                                                     & 75\%                                                                 & 14.152                                                            & 0.660                                             & 0.702                         & 0.587                                                               & 0.588                         & 0.484                         & 0.488                                                                     & 0.589                         \\

\multirow{-2}{*}{\textbf{RAP}}                                                       & 50\%                                                                 & 18.540                                                            & 0.309                                             & 0.618                         & 0.533                                                               & 0.438                         & 0.435                         & 0.302                                                                     & 0.460                         \\ \hdashline
                                                                                     & \cellcolor[HTML]{EFEFEF}75\%                                         & \cellcolor[HTML]{EFEFEF}14.520                                    & \cellcolor[HTML]{EFEFEF}0.616                     & \cellcolor[HTML]{EFEFEF}0.700 & \cellcolor[HTML]{EFEFEF}0.578                                       & \cellcolor[HTML]{EFEFEF}0.590 & \cellcolor[HTML]{EFEFEF}0.457 & \cellcolor[HTML]{EFEFEF}0.493                                             & \cellcolor[HTML]{EFEFEF}0.584 \\
\multirow{-2}{*}{\textbf{Ours}}                                                      & 50\%                                                                 & 16.016                                                            & 0.499                                             & 0.644                         & 0.542                                                               & 0.531                         & 0.454                         & 0.400                                                                     & 0.521                         \\ \hline
\end{tabular}
}
\end{table}

==> tables/table1_baseline_comparisons.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{
\textbf{Comparison of methods that compress KV Cache along head dimension.}
RACE operates natively in the reduced dimensions without reconstruction.
See ~\ref{app:table1_derivation} for the derivations.
}
% \vspace{0.3cm}
\label{tab:flops_analysis}
\resizebox{\columnwidth}{!}{%

\begin{tabular}{ccccccccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Method} & \textbf{\begin{tabular}[c]{@{}c@{}}Recons-\\ truction\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Calibration\\  Signal\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Custom\\  Kernel\end{tabular}} &\textbf{\begin{tabular}[c]{@{}c@{}}Compression\\ Criterion (Q/K)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}KV Cache \\ Retained\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Attn. Params\\  Retained\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prefill \\ FLOPs\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Decoding\\  FLOPs\end{tabular}} \\ \hline
Full Attention \cite{attention} & -                                                                     & -                                                                    &No    & -                                                                           & 100\%                                                                 & 100\%                                                                     & 1 X                                                               & 1 X                                                                \\
\rowcolor[HTML]{EFEFEF} 
EigenAttention \cite{saxena2024eigen}  & Yes                                                                   & Activations                                                     &No       & Truncated SVD                                                                         & 50\%                                                                  & 64.6\%                                                                    & 0.75 X                                                            & 32.75 X                                                            \\
PALU    \cite{chang2025palu}        & Yes                                                                   & Weights                                                            & Yes     & Truncated SVD                                                                         & 50\%                                                                  & 66.7\%                                                                    & 0.75 X                                                            & 64.75 X                                                                                    \\
\rowcolor[HTML]{EFEFEF} 
Thin Keys  \cite{thinkeys}      & No                                                                    & Weights                                                             &No     & Truncated SVD                                                                         & 75\%                                                                  & 50\%                                                                      & 0.75 X                                                            & 0.75 X                                                             \\

RAP  \cite{rap}           & No                                                                  & Gradients             &No                                                     & Fisher Pruning                                                                     & 50\%                                                                  & 50\%                                                                      & 0.5 X                                                             & 0.5 X                                                              \\
\rowcolor[HTML]{EFEFEF} 
\textbf{RACE}(Ours)            & No                                                                    & Activations                                                        &No      & Pair Energy Sel.                                                               & 50\%                                                                  & 50\%                                                                      & 0.5 X                                                             & 0.5 X                                                              \\ \hline
\end{tabular}
}

\end{table}


